On Inductive Biases for Machine Learning in Data Constrained Settings

Learning with limited data is one of the biggest problems of machine learning. Current approaches to this issue consist in learning general representations from huge amounts of data before fine-tuning the model on a small dataset of interest. While such technique, coined transfer learning, is very effective in domains such as computer vision or natural langage processing, it does not yet solve common problems of deep learning such as model interpretability or the overall need for data. This thesis explores a different answer to the problem of learning expressive models in data constrained settings: instead of relying on big datasets to learn neural networks, we will replace some modules by known functions reflecting the structure of the data. Very often, these functions will be drawn from the rich literature of kernel methods. Indeed, many kernels can reflect the underlying structure of the data, thus sparing learning parameters to some extent. Our approach falls under the hood of "inductive biases", which can be defined as hypothesis on the data at hand restricting the space of models to explore during learning. We demonstrate the effectiveness of this approach in the context of sequences, such as sentences in natural language or protein sequences, and graphs, such as molecules. We also highlight the relationship between our work and recent advances in deep learning. Additionally, we study convex machine learning models. Here, rather than proposing new models, we wonder which proportion of the samples in a dataset is really needed to learn a "good" model. More precisely, we study the problem of safe sample screening, i.e, executing simple tests to discard uninformative samples from a dataset even before fitting a machine learning model, without affecting the optimal model. Such techniques can be used to prune datasets or mine for rare samples.

==> chapters/2_samplescreening/ellipsoid.tex <==
A subgradient of the \ref{s-lasso_pb} objective in $x$ is:
\begin{align*}
    A^t \ell'(Ax - b) + \lambda v_2
\end{align*}
with 
\begin{displaymath}
\ell'_i(u) \begin{cases}
            = 2 (u_i - \text{sgn}(u_i) \mu) & \text{if } |u_i| > \mu, \\
            = 0 & \text{otherwise}
            \end{cases}
            \end{displaymath}
and 
\begin{displaymath}
v_2^i(u) \begin{cases}
               = \text{sgn}(u_i) & \text{if } u_i \neq 0,\\
                \in [-1,1] & \text{otherwise}.
               \end{cases}
            \end{displaymath}


==> chapters/graphit/add_vis.tex <==
\section{Additional visualization of Mutagenicity compounds}
\label{sec:add_vis}

In this section, we use attention scores as a visualization mechanism for detecting substructures that may possibly induce mutagenicity. We apply our model to samples from the Mutagenicity data set~\cite{KKMMN2016} and analyze molecules that were correctly classified as mutagenic.

\paragraph{1,2-Dibromo-3-Chloropropane (DBCP).} 
DBCP in Figure~\ref{fig:dbcp} was used as a soil fumigant in various countries. It was banned from use in the United Stated in 1979 after evidences that DBCP causes diseases, male sterility, or blindness, which can be instances of mutagenicity. In Figure~\ref{fig:attentions_dbcp}, attention focuses on the carbon skeleton and on the two Bromine (Br) atoms, the latter being indeed known for being associated with mutagenicity~\cite{LAG199473}.


%\begin{figure}
%\centering
%\includegraphics[scale=0.8]{figures/origin2012.pdf}
%\caption{1,2-Dibromo-3-Chloropropane.}
%\label{fig:dbcp}
%\end{figure}

\begin{figure}
\centering
\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[scale=0.5]{chapters/graphit/figures/colorbar_appendix.pdf}
\end{subfigure}

\vspace{1cm}

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[scale=1.0]{chapters/graphit/figures/origin2012.pdf}
\end{subfigure}
\caption{1,2-Dibromo-3-Chloropropane.}
\label{fig:dbcp}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1\linewidth]{chapters/graphit/figures/attns_2012_1_t.pdf}
\end{subfigure}

\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1\linewidth]{chapters/graphit/figures/attns_2012_2_t.pdf}
\end{subfigure}

\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1\linewidth]{chapters/graphit/figures/attns_2012_3_t.pdf}
\end{subfigure}

\caption{Attention scores averaged by heads for each layer of our trained model for the compound in Figure~\ref{fig:dbcp}. \textit{Left}: diffusion kernel for~\ref{fig:dbcp}.  \textit{Right}: node $3$ and $5$ (Br) are salient.}
\label{fig:attentions_dbcp}
\end{figure}

\paragraph{Nitrobenzene-nitroimidazothiazole.} This compound is shown in Figure~\ref{fig:2NO2}. As for compound~\ref{fig:NO2} in Section~\ref{subsec:visu}, our model puts emphasis on two nitro groups which are indeed known for inducing mutagenicity.

\begin{figure}
\centering
\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[scale=0.35]{chapters/graphit/figures/colorbar_appendix.pdf}
\end{subfigure}

\vspace{1cm}

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[scale=0.8]{chapters/graphit/figures/origin2010.pdf}
\end{subfigure}
\caption{Nitrobenzene-nitroimidazothiazole.}
\label{fig:2NO2}
\end{figure}

%\begin{figure}
%\centering
%\includegraphics[scale=0.8]{figures/origin2010.pdf}
%\caption{Nitrobenzene-nitro-hexahydroimidazo-thiazole.}
%\label{fig:2NO2}
%\end{figure}

\begin{figure}
\centering

\begin{subfigure}{1.0\textwidth}
    \includegraphics[width = 1.6in]{chapters/graphit/figures/attns_2010_1_t.pdf}
\end{subfigure}

\begin{subfigure}{1.0\textwidth}
    \includegraphics[width = 1.6in]{chapters/graphit/figures/attns_2010_2_t.pdf}
\end{subfigure}

\begin{subfigure}{1.0\textwidth}
    \includegraphics[width = 1.6in]{chapters/graphit/figures/attns_2010_3_t.pdf}
\end{subfigure}

\caption{Attention scores averaged by heads for each layer of our trained model for the compound in Figure~\ref{fig:2NO2}. \textit{Left}: diffusion kernel for~\ref{fig:2NO2}.  \textit{Right}: node $5$ and $17$ (N) are salient.}
\label{fig:attentions_2NO2}
\end{figure}

%\paragraph{Chloroethylcarbamoylesulfide-purine.} Our model puts emphasis on remarkable atoms: Sulfur (S), Nitrogen (N), and Chlorine (Cl). To the best of our knowledge in chemistry, their role as mutagenicity-inducing groups is unclear for this compound, perhaps suggesting the interest of further studying the influence of these groups.

%\begin{figure}
%\centering
%\begin{subfigure}{1.0\textwidth}
%\centering
%\includegraphics[scale=0.35]{figures/colorbar_appendix.pdf}
%\end{subfigure}

%\vspace{1cm}

%\begin{subfigure}{1.0\textwidth}
%\centering
%\includegraphics[scale=0.8]{figures/origin2005.pdf}
%\end{subfigure}
%\caption{Chloroethylcarbamoylesulfide-purine.}
%\label{fig:purine}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[scale=0.8]{figures/origin2005.pdf}
%\caption{Chloroethylcarbamoyd-sulfur-purine.}
%\label{fig:purine}
%\end{figure}

%\begin{figure}
%\centering
%\begin{tabular}{ccc}
%\subfloat{\includegraphics[width = 1.6in]{figures/attns_2005_1_t.pdf}} &
%\subfloat{\includegraphics[width = 1.6in]{figures/attns_2005_2_t.pdf}} &
%\subfloat{\includegraphics[width = 1.6in]{figures/attns_2005_3_t.pdf}}\\
%\end{tabular}
%\caption{Attention scores averaged by heads for each layer of our trained model for the compound in Figure~\ref{fig:purine}. \textit{Left}: diffusion kernel for~\ref{fig:purine}.  \textit{Right}: node $3$ and $5$ (Br) are salient.}
%\label{fig:attentions_purine}
%\end{figure}

\paragraph{Triethylenemelamine.} Triethylenemelamine in Figure~\ref{fig:tmel} is a compound exhibiting mutagenic properties, and is used to induce cancer in experimental animal models. Our model focuses on the three nitrogen atoms of the aziridine groups which are themselves mutagenic compounds.

\begin{figure}
\centering
\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[scale=0.35]{chapters/graphit/figures/colorbar_appendix.pdf}
\end{subfigure}

\vspace{1cm}

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[scale=0.8]{chapters/graphit/figures/origin2029.pdf}
\end{subfigure}
\caption{Triethylenemelamine.}
\label{fig:tmel}
\end{figure}

%\begin{figure}
%\centering
%\includegraphics[scale=0.8]{figures/origin2005.pdf}
%\caption{Chloroethylcarbamoyd-sulfur-purine.}
%\label{fig:purine}
%\end{figure}

\begin{figure}
\centering

\begin{subfigure}{1.0\textwidth}
    \includegraphics[width = 1.6in]{chapters/graphit/figures/attns_2029_1_t.pdf}
\end{subfigure}

\begin{subfigure}{1.0\textwidth}
    \includegraphics[width = 1.6in]{chapters/graphit/figures/attns_2029_2_t.pdf}
\end{subfigure}

\begin{subfigure}{1.0\textwidth}
    \includegraphics[width = 1.6in]{chapters/graphit/figures/attns_2029_3_t.pdf}
\end{subfigure}

\caption{Attention scores averaged by heads for each layer of our trained model for the compound in Figure~\ref{fig:tmel}. \textit{Left}: diffusion kernel for~\ref{fig:tmel}.  \textit{Right}: node $1$, $8$, and $10$ (N) are salient.}
\label{fig:attentions_tmel}
\end{figure}


==> chapters/otke/add_background.tex <==
\subsection{Attention and transformers} We clarify the concept of attention --- a mechanism yielding a context-dependent embedding for each element of $\mathbf{x}$ --- as a special case of non-local operations~\citep{Wang2017, Buades2011}, so that it is easier to understand its relationship to the OTK. Let us assume we are given a set $\mathbf{x} \in \mathcal{X}$ of length $n$. A non-local operation on $\mathbf{x}$ is a function $\Phi: \mathcal{X} \mapsto \mathcal{X}$ such that
\begin{equation*}
    \Phi(\mathbf{x})_i = \sum_{j=1}^{n} w(\mathbf{x}_i, \mathbf{x}_j) v(\mathbf{x}_j)=\mathbf{W}(\mathbf{x})_i^{\top} \mathbf{V}(\mathbf{x}),
\end{equation*}
where $\mathbf{W}(\mathbf{x})_i$ denotes the $i$-th column of $\mathbf{W}(\mathbf{x})$, a weighting function, and $\mathbf{V}(\mathbf{x}) = [v(\mathbf{x}_1), \dots, v(\mathbf{x}_n)]^\top$, an embedding. In contrast to operations on local neighborhood such as convolutions, non-local operations theoretically account for long range dependencies between elements in the set. In attention and the context of neural networks, $w$ is a \textit{learned} function reflecting the \textit{relevance} of each other elements $\mathbf{x}_j$ with respect to the element $\mathbf{x}_i$ being embedded and given the task at hand. In the context of the chapter, we compare to a type of attention coined as \textit{dot-product self-attention}, which can typically be found in the encoder part of the transformer architecture ~\citep{vaswani2017}. Transformers are neural network models relying mostly on a succession of an attention layer followed by a fully-connected layer. Transformers can be used in sequence-to-sequence tasks --- in this setting, they have an encoder with self-attention and a decoder part with a variant of self-attention ---, or in sequence to label tasks, with only the encoder part. The chapter deals with the latter. The name self-attention means that the attention is computed using a dot-product of linear transformations of $\mathbf{x}_i$ and $\mathbf{x}_j$, and $\mathbf{x}$ attends to itself only. In its matrix formulation, dot-product self-attention is a non-local operation whose matching vector is
\begin{equation*}
    \mathbf{W}(\mathbf{x})_i = \text{Softmax}\left( \frac{W_Q \mathbf{x}_i \mathbf{x}^\top W_K^\top}{\sqrt{d_k}} \right),
    \label{eq:attention}
\end{equation*}
where $W_Q \in \Real^{n \times d_k}$ and $W_K \in \Real^{n \times d_k}$ are learned by the network.
In order to know which $\mathbf{x}_j$ are relevant to $\mathbf{x}_i$, the network computes scores between a query for $\mathbf{x}_i$ ($W_Q \mathbf{x}_i$) and keys of all the elements of $\mathbf{x}$ ($W_K \mathbf{x}$). The softmax turns the scores into a weight vector in the simplex. Moreover, a linear mapping $\mathbf{V}(\mathbf{x}) = W_V \mathbf{x}$, the values, is also learned.  $W_Q$ and $W_K$ are often shared \citep{kitaev2020reformer}. A drawback of such attention is that for a sequence of length $n$, the model has to store an attention matrix $\mathbf{W}$ with size $O(n^2)$. More details can be found in~\cite{vaswani2017}. %A transformer architecture has multiples heads, \textit{i.e} alternances between attention mechanisms and fully-connected layers, in parrallel. %The resulting embeddings are then concatenated and multiplied by another weight matrix (learned). 
%Crucially, because attention does not keep track of the position of the elements, a transformer encodes the position of the elements in the sequence and adds it to the initial embedding. %Interestingly, there is no paper using the same embedding for $Q$, $K$ and $V$.


==> defsperms.tex <==
% Permutation related sets and notations
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cPH}{\mathcal{PH}}
\providecommand{\PAP}{\Pi A \Pi^T}
% (Strong ?) Robinson and circular Robinson
\providecommand{\cR}{\mathcal{L}_{R}}
\providecommand{\circR}{\mathcal{C}_{R}}
% Miscellaneous
\providecommand{\cZ}{\mathcal{Z}}
\providecommand{\cSN}{\mathcal{SN}}
% Manifold
\providecommand{\cM}{\mathcal{M}}
% Hyperplane
\providecommand{\cH}{\mathcal{H}}
% Normalized Laplacians
\providecommand{\Lrw}{L^{\text{rw}}}
\providecommand{\Lsym}{L^{\text{sym}}}
%k-dimensional Lapl. embedding
\providecommand{\kLE}[1]{#1-$\mathbf{LE}$}
% Symmetric Circulant Robinson
\providecommand{\SCR}{\mathcal{C}_{R}^*}

%\providecommand{\st}{\ensuremath{\textrm{s.t.}\quad}}
\providecommand{\st}{\text{such that}}
\providecommand{\find}{\text{find}}

\newcommand{\argsort}{\mathop{\rm argsort}}
